Who2com: Collaborative Perception via Learnable Handshake Communication

In this paper, we propose the problem of collaborative perception, where robots can combine their local observations with those of neighboring agents in a learnable way to improve accuracy on a perception task. Unlike existing work in robotics and multi-agent reinforcement learning, we formulate the problem as one where learned information must be shared across a set of agents in a bandwidth-sensitive manner to optimize for scene understanding tasks such as semantic segmentation. Inspired by networking communication protocols, we propose a multi-stage handshake communication mechanism where the neural network can learn to compress relevant information needed for each stage. Specifically, a target agent with degraded sensor data sends a compressed request, the other agents respond with matching scores, and the target agent determines who to connect with (i.e., receive information from). We additionally develop the AirSim-CP dataset and metrics based on the AirSim simulator where a group of aerial robots perceive diverse landscapes, such as roads, grasslands, buildings, etc. We show that for the semantic segmentation task, our handshake communication method significantly improves accuracy by approximately 20% over decentralized baselines, and is comparable to centralized ones using a quarter of the bandwidth.

==> table/case_description.tex <==



\begin{table*}
\caption{
\textbf{Comparison of our experimental cases.} 
Additional details and qualitative examples are in the Appendix.
}
\label{tab:case}
\centering
% \small
% \scriptsize
% \footnotesize
% \tiny
\scriptsize{
\begin{tabular}{cccc}
\toprule
& Case 1 & Case 2 & Case 3 (Sanity check) \\
\midrule
Geometric warping & Yes & No & No \\
Target agent & Fixed & Fixed & Random \\
Normal agents & Fixed & Fixed & Shuffled \\
Overlapping FOVs & Partial & Complete & Complete \\
% Training samples &  9,515&  9,490&  9,490\\
% Validation samples & 2,735 & 2,980 &  2,980\\
% Testing samples & 4,080 & 4,270 & 4,270 \\
\midrule
% Challenge & Partial overlap FOVs& Non-warped observations & Random target \\
\multirow{2}{*}{ Challenge(s) } & \multirow{2}{*}{ Partially overlapping FOVs  } & \multirow{2}{*}{ Non-warped confusers } & Non-warped images \\
& & & Random target \\

\bottomrule
\end{tabular}}
\end{table*}


==> table/table_attention_ablation.tex <==
\begin{table}
\caption{\textbf{A comparison of different attention mechanisms.} Note that 8-1024 represents the model with the message size of $8$ and the key size of $1024$. The general attention mechanism achieves the best performance under the same bandwidth condition. }
\label{tab:ablation}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
& Scale-Dot (8-8) & Additive(8-1024) & General (8-8)& General (8-1024) & w/o message 
\\ \midrule
Selection Accuracy($\%$) & 59.02 & 37.7 & 59.48 & \textbf{95.9} & 25.52\\
Mean IoU($\%$) & 38.39 & 33.79 & 38.88 & \textbf{49.59} & 32.25\\
\bottomrule
%\label{tab:ablation}
\end{tabular}}
\end{table}


==> table/table_resnet_case5.tex <==


\begin{table*}
\caption{\textbf{Experimental results on case 2.} Our method achieve competitive performance and significant better IBS compared to the centralized methods in the case of no geometric warping of the views.} 
\label{tab:res_case5}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
& & Overall Acc & Mean Acc & FreqW Acc & Mean IoU & Bandwidth (in kbpf) & IBS\\
\midrule
Upper bound & Single Normal & 89.55$\pm$0.07 & 61.69$\pm$0.12 & 82.04$\pm$0.11 & 52.39$\pm$0.08 & & \\
\midrule
\multirow{2}{*}{Centralized} & CatAll & 83.29$\pm$0.12 & 46.22$\pm$0.07 & 72.73$\pm$0.1 & 39.38$\pm$0.12 & 4096& 1.66\\
& Weight sum & 89.46$\pm$0.07 & 60.28$\pm$0.1 & 81.81$\pm$0.1 & 51.8$\pm$0.22 & 4096.03 & 3.20\\
% & Ours w/ msg (Softmax) & 89.39$\pm$0.11 & 60.21$\pm$0.03 & 81.75$\pm$0.11 & 51.31$\pm$0.13 & 4100.03& 3.17 \\
\midrule
\multirow{3}{*}{ Distributed } 
& Random Selection & 77.58$\pm$0.77 & 42.76$\pm$0.38 & 65.31$\pm$0.96 & 34.6$\pm$0.67 & 1024 & 0.92\\
& Ours w/o msg  & 89.43$\pm$0.08 & 60.28$\pm$0.09 & 81.78$\pm$0.11 & 51.74$\pm$0.25 & 1024.03 & \textbf{12.77}\\
& Ours w/ msg & 89.37$\pm$0.13 & 60.2$\pm$0.04 & 81.73$\pm$0.15 & 51.3$\pm$0.14 & 1028.03 & 12.66\\
\midrule
Lower bound & Single Degraded & 76.66$\pm$0.2 & 41.72$\pm$0.44 & 64.28$\pm$0.13 & 33.63$\pm$0.22 & & \\
\bottomrule
\end{tabular}}
\end{table*}


==> table/table_resnet_htv.tex <==


\begin{table}[t!]
\caption{\textbf{Experimental results on Hidden Target View case.} Comparing \textit{Ours w/o msg} with \textit{Ours w/ msg} demonstrates the importance of the message $\bm{\mu}_{j}$ for this case. }
\label{tab:res_case6}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
& & Overall Acc  & BW (kbpf) & BIS \\\midrule
Upper bound & Single Normal & 88.14$\pm$0.02   & & \\\midrule
\multirow{3}{*}{Centralized }
& CatAll & 72.58$\pm$0.14 & 4096 & 0.049\\

& Attention & 69.08$\pm$0.76  &  4096.03 & 0.004\\
& Compression & 70.44 &  1024 & 0.085\\

% & Ours w/ msg (Softmax) & 84.72$\pm$0.49 & 57.36$\pm$0.56 & 73.79$\pm$0.77 & 49.37$\pm$0.53 & 4100.03 & 3.98\\
\midrule
\multirow{3}{*}{ Distributed }
& Random Selection & 69.16$\pm$0.19  & 1024 & 0.019\\
& \textbf{Ours w/o msg}  & 65.31$\pm$0.22  & 1024.03 & -0.179\\
& \textbf{Ours w/ msg}  & \textbf{84.57$\pm$0.62}  &  1028.03 & \textbf{0.812}\\
\midrule
Lower bound & Single Degraded & 68.79$\pm$0.59  &   & \\
\bottomrule



\end{tabular}}
\end{table}




% \begin{table}[t!]
% \caption{\textbf{Experimental results on Hidden Target View case.} Our method with message achieves better performance and BIS compared to the centralized methods. Comparing \textit{Ours w/o msg} with \textit{Ours w/ msg} demonstrates the importance of the message $\bm{\mu}_{j}$ in the case of shuffled degraded agent. }
% \label{tab:res_case6}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{cccccc}
% \toprule
% & & Overall Acc  & Mean IoU & BW (kbpf) & BIS \\\midrule
% Upper bound & Single Normal & 88.14$\pm$0.02  & 53.74$\pm$0.08 & & \\\midrule
% \multirow{3}{*}{Centralized }
% & CatAll & 72.58$\pm$0.14 & 38.0$\pm$0.05 & 4096 & 0.049\\
% % & CatAll(16-16-128) & 70.20$\pm$0.90 & 44.05$\pm$0.50 & 54.61$\pm$0.70 & 35.87$\pm$0.51 & 1028.03 & \textcolor{red}{1.01}\\
% % & CatAll(8-8-512) & 70.44$\pm$0.67 & 44.26$\pm$0.57 & 54.69$\pm$0.87 & 35.81$\pm$0.52 & 1028.03 & \textcolor{red}{0.95}\\

% & Attention & 69.08$\pm$0.76  & 35.25$\pm$0.53 & 4096.03 & 0.004\\
% & \textcolor{red}{Compression} & 70.44 &  35.81 & 1024 & 0.085\\

% % & Ours w/ msg (Softmax) & 84.72$\pm$0.49 & 57.36$\pm$0.56 & 73.79$\pm$0.77 & 49.37$\pm$0.53 & 4100.03 & 3.98\\
% \midrule
% \multirow{3}{*}{ Distributed }
% & Random Selection & 69.16$\pm$0.19  & 35.22$\pm$0.05 & 1024 & 0.019\\
% & \textbf{Ours w/o msg}  & 65.31$\pm$0.22  & 32.36$\pm$0.38 & 1024.03 & -0.179\\
% & \textbf{Ours w/ msg}  & \textbf{84.57$\pm$0.62}  & \textbf{49.15$\pm$0.68} & 1028.03 & \textbf{0.812}\\
% \midrule
% Lower bound & Single Degraded & 68.79$\pm$0.59  & 34.86$\pm$0.26 &  & \\
% \bottomrule



% \end{tabular}}
% \end{table}


==> table/table_resnet_nav_ip.tex <==
\begin{table}
\caption{\textbf{Experimental results on Multi-agent Navigation (inaccurate pose).} Our method achieve competitive accuracy and significant better BIS compared to the centralized methods in the case of partial overlapping field of views.}
\label{tab:res_nav_ip}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
& & Overall Acc & BW (kbpf) & BIS \\
\midrule
Upper bound & Single Normal & 89.7$\pm$0.04  &  &\\
\midrule
\multirow{2}{*}{Centralized } & CatAll & 80.33$\pm$0.6  & 4096 & 0.172\\
& Attention & 82.79$\pm$0.16  & 4096.03 & 0.174\\
& Compression & 76.93  & 1024 & 0.441\\
\midrule
\multirow{3}{*}{ Distributed }
& Random Selection & 67.49$\pm$1.12  & 1024 & 0.028\\
& Ours w/o msg & 79.34$\pm$0.06  & 1024.03 & 0.546\\
& Ours w/ msg & 79.44$\pm$0.14  & 1028.03 & \textbf{0.549}\\
\midrule
Lower bound & Single Degraded & 66.84$\pm$0.03 &  & \\
\bottomrule
\end{tabular}}
\end{table}


% \begin{table}
% \caption{\textbf{Experimental results on Multi-agent Navigation (inaccurate pose).} Our method achieve competitive accuracy and significant better BIS compared to the centralized methods in the case of partial overlapping field of views.}
% \label{tab:res_nav_ip}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{cccccc}
% \toprule
% & & Overall Acc & Mean IoU & BW (kbpf) & BIS \\
% \midrule
% Upper bound & Single Normal & 89.7$\pm$0.04  & 46.48$\pm$0.1 & &\\
% \midrule
% \multirow{2}{*}{Centralized } & CatAll & 80.33$\pm$0.6  & 33.13$\pm$0.56 & 4096 & 0.172\\
% & Attention & 82.79$\pm$0.16  & 35.43$\pm$0.13 & 4096.03 & 0.174\\
% % & Ours w/ msg (Softmax) & 82.86$\pm$0.05 & 42.66$\pm$0.41 & 70.86$\pm$0.06 & 35.62$\pm$0.12 & 4100.03 & 4.00 \\
% \midrule
% \multirow{3}{*}{ Distributed }
% & Random Selection & 67.49$\pm$1.12  & 23.35$\pm$0.76 & 1024 & 0.028\\
% & Ours w/o msg & 79.34$\pm$0.06  & 32.86$\pm$0.08 & 1024.03 & 0.546\\
% & Ours w/ msg & 79.44$\pm$0.14  & 32.8$\pm$0.08 & 1028.03 & \textbf{0.549}\\
% \midrule
% Lower bound & Single Degraded & 66.84$\pm$0.03 & 22.73$\pm$0.1 & & \\
% \bottomrule
% \end{tabular}}
% \end{table}

==> table/table_resnet_nav_p.tex <==
% \begin{table}
% \caption{\textbf{Experimental results on Multi-agent Navigation (accurate pose).}}
% \label{tab:res_nav_p}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{cccccc}
% \toprule
% & & Overall Acc & Mean IoU & BW (kbpf) & BIS \\
% \midrule
% Upper bound & Single Normal & 88.13  & 53.76 & &\\
% \midrule
% \multirow{2}{*}{Centralized } & CatAll & 80.05  & 40.54 & 4096 & 0.17\\
% & Attention & 84.38  & 46.48 & 4096.03 & 0.212\\
% % & Ours w/ msg (Softmax) & 82.86$\pm$0.05 & 42.66$\pm$0.41 & 70.86$\pm$0.06 & 35.62$\pm$0.12 & 4100.03 & 4.00 \\
% \midrule
% \multirow{3}{*}{ Distributed }
% & Random Selection & 64.94  & 27.22 & 1024 & 0.082\\
% & Ours w/o msg & 78.10  & 40.52 & 1024.03 & 0.602\\
% & Ours w/ msg & 80.42  & 41.37 & 1028.03 & \textbf{0.691}\\
% \midrule
% Lower bound & Single Degraded & 62.88 & 25.42 & & \\
% \bottomrule
% \end{tabular}}
% \end{table}


\begin{table}
\caption{\textbf{Experimental results on Multi-agent Navigation (accurate pose).}}
\label{tab:res_nav_p}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
& & Overall Acc & BW (kbpf) & BIS \\
\midrule
Upper bound & Single Normal & 88.13  &  &\\
\midrule
\multirow{3}{*}{Centralized } & CatAll & 80.05  & 4096 & 0.17\\
& Attention & 84.38  & 4096.03 & 0.212\\
& Compression & 76.2  & 1024 & 0.527\\
\midrule
\multirow{3}{*}{ Distributed }
& Random Selection & 64.94  & 1024 & 0.082\\
& Ours w/o msg & 78.10  & 1024.03 & 0.602\\
& Ours w/ msg & 80.42  & 1028.03 & \textbf{0.691}\\
\midrule
Lower bound & Single Degraded & 62.88 &  & \\
\bottomrule
\end{tabular}}
\end{table}

==> table/table_resnet_search.tex <==
% \begin{table}
% \caption{\textbf{Experimental results on Multi-agent Visual Search.} Our method achieve competitive accuracy and significant better BIS compared to the centralized methods in the case of partial overlapping field of views.}
% \label{tab:res_search}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{cccccc}
% \toprule
% & & Overall Acc & Mean IoU & BW (kbpf) & BIS \\
% \midrule
% Upper bound & Single Normal &  89.16 & 50.51 & &\\
% \midrule
% \multirow{3}{*}{Centralized } & CatAll & 78.74  & 31.09 & 4096 & 0.133 \\
% & Attention &  81.07 & 34.20 & 4096.03 & 0.159 \\
% & Compression &  76.18 & 27.39 & 1024 & 0.418\\
% % & Ours w/ msg (Softmax) & 82.86$\pm$0.05 & 42.66$\pm$0.41 & 70.86$\pm$0.06 & 35.62$\pm$0.12 & 4100.03 & 4.00 \\
% \midrule
% \multirow{3}{*}{ Distributed }
% & Random Selection & 69.58  & 20.87 & 1024 & 0.123 \\
% & Ours w/o msg &  80.69 & 33.53 & 1024.03 & 0.621\\
% & \textbf{Ours w/ msg} & 80.97  & 33.91 & 1028.03 & \textbf{0.631}\\
% \midrule
% Lower bound & Single Degraded & 66.84 & 19.86 & & \\
% \bottomrule
% \end{tabular}}
% \end{table}


\begin{table}
\caption{\textbf{Experimental results on Multi-agent Visual Search.} Our method achieve competitive accuracy and significantly better BIS compared to the centralized methods.}
\label{tab:res_search}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccc}
\toprule
& & Overall Acc & BW (kbpf) & BIS \\
\midrule
Upper bound & Single Normal &  89.16 & -  & - \\
\midrule
\multirow{3}{*}{Centralized } & CatAll & 78.74  & 4096 & 0.133 \\
& Attention &  81.07 & 4096.03 & 0.159 \\
& Compression &  73.05 & 1024 & 0.277\\
\midrule
\multirow{3}{*}{ Distributed }
& Random Selection & 69.58  & 1024 & 0.123 \\
& Ours w/o msg &  80.69 & 1024.03 & 0.621\\
& \textbf{Ours w/ msg} & \textbf{80.97}  & 1028.03 & \textbf{0.631}\\
\midrule
Lower bound & Single Degraded & 66.84 & - & - \\
\bottomrule
\end{tabular}}
\end{table}


==> table/table_segnet_case4.tex <==
\begin{table}
\caption{\textbf{Evaluation on testing set of case4 with SegNet.} }
\label{tab:seg_case4}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccc}
\toprule
& & Overall Acc & Mean Acc & FreqW Acc & Mean IoU & Bandwidth (Kbytpes per frame) \\ \midrule
Upper bound & Single Normal image & 83.46$\pm$0.13 & 41.83$\pm$0.16 & 72.21$\pm$0.1 & 35.96$\pm$0.08 & \\ \midrule
\multirow{3}{*}{ Fully Centralized } & Concatenates all features & 75.53$\pm$0.16 & 36.49$\pm$0.45 & 61.58$\pm$0.02 & 29.28$\pm$0.17 & 256 \\
& Detached Encoder w/ msg (Weighted Sum) & 79.17$\pm$0.16 & 38.85$\pm$0.22 & 66.14$\pm$0.25 & 32.0$\pm$0.14 & 64.28 \\
& Detached Encoder w/o msg (Weighted Sum) & & & & & 64.03 \\\midrule
\multirow{5}{*}{ Distributed } & Random Selection & 61.23$\pm$1.01 & 29.11$\pm$0.31 & 46.46$\pm$0.78 & 21.27$\pm$0.33 & 64 \\
& Detached Encoder w/o msg (Argmax Test) & & & & & 64.03 \\
& Detached Encoder w/o msg (2-head decoder) & & & & & 64.03 \\
& Detached Encoder (Argmax Test) & 75.94$\pm$0.09 & 36.56$\pm$0.21 & 61.92$\pm$0.16 & 29.61$\pm$0.14 & 64.28 \\
& Detached Encoder (2-head decoder) & 76.84$\pm$0.19 & 37.36$\pm$0.18 & 63.08$\pm$0.09 & 30.31$\pm$0.07 & 64.28 \\\midrule
Lower bound & Single Degraded image & 60.04$\pm$0.64 & 27.15$\pm$0.36 & 44.04$\pm$0.76 & 19.99$\pm$0.43 & \\
\bottomrule
\end{tabular}}
\end{table}



==> table/table_segnet_case5.tex <==


\begin{table}
\caption{\textbf{Evaluation on testing set of case5 with SegNet.} }
\label{tab:seg_case5}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccc}
\toprule
& & Overall Acc & Mean Acc & FreqW Acc & Mean IoU & Bandwidth (Kbytpes per frame) \\ \midrule
Upper bound & Single Normal image & 82.81$\pm$0.15 & 46.78$\pm$0.27 & 72.4$\pm$0.13 & 38.38$\pm$0.29 & \\\midrule
\multirow{3}{*}{ Fully Centralized } & Concatenates all features & 73.37$\pm$0.46 & 35.73$\pm$0.28 & 59.91$\pm$0.61 & 27.79$\pm$0.34 & 256 \\
& Detached Encoder w/ msg (Weighted Sum) & 83.01$\pm$0.11 & 46.27$\pm$1.04 & 72.6$\pm$0.14 & 37.98$\pm$0.8 & 64.28 \\
& Detached Encoder w/o msg (Weighted Sum) & 83.02$\pm$0.28 & 45.76$\pm$0.53 & 72.84$\pm$0.3 & 37.6$\pm$0.24 & 64.03 \\ \midrule
\multirow{5}{*}{ Distributed }& Random Selection & 70.73$\pm$0.21 & 33.51$\pm$0.43 & 57.23$\pm$0.02 & 25.89$\pm$0.14 & 64 \\
& Detached Encoder w/o msg (Argmax Test) & 82.98$\pm$0.31 & 45.75$\pm$0.49 & 72.79$\pm$0.34 & 37.56$\pm$0.24 & 64.03 \\
& Detached Encoder w/o msg (2-head decoder) & 83.1$\pm$0.11 & 44.68$\pm$0.42 & 72.91$\pm$0.27 & 37.12$\pm$0.27 & 64.03 \\
& Detached Encoder (Argmax Test) & 82.97$\pm$0.11 & 46.26$\pm$1.05 & 72.56$\pm$0.13 & 37.96$\pm$0.82 & 64.28 \\
& Detached Encoder (2-head decoder) & 83.04$\pm$0.08 & 45.67$\pm$1.23 & 72.59$\pm$0.11 & 37.92$\pm$0.95 & 64.28 \\ \midrule
Lower bound & Single Degraded image & 70.47$\pm$0.19 & 33.19$\pm$0.18 & 56.65$\pm$0.21 & 25.51$\pm$0.08 & \\
\bottomrule
\end{tabular}}
\end{table}


==> table/table_segnet_case6.tex <==
\begin{table}
\caption{\textbf{Evaluation on testing set of case6 with SegNet.} }
\label{tab:seg_case6}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccc}
\toprule
& & Overall Acc & Mean Acc & FreqW Acc & Mean IoU & Total (in Kbytpes per frame) \\\midrule
Upper bound & Single Normal image & 78.74 & 47.36 & 65.69 & 39.02 & \\\midrule
\multirow{3}{*}{ Fully Centralized } & Concatenates all features & 65.69 & 37.23 & 49.26 & 28.64 & 256 \\
& Our model w/ msg (Weighted Sum) & 75.98$\pm$0.11 & 45.99$\pm$0.34 & 61.93$\pm$0.18 & 37.29$\pm$0.32 & 256.28 \\
& Our model w/o msg (Weighted Sum) & 66.31$\pm$0.22 & 35.29$\pm$0.47 & 50.0$\pm$0.18 & 27.89$\pm$0.56 & 256.03 \\\midrule
\multirow{5}{*}{ Distributed }& Random Selection & 62.4 & 36.07 & 46.27 & 27.43 & 64 \\
& Our model w/o msg (Argmax Test)  & 61.41$\pm$0.32 & 33.05$\pm$0.29 & 45.56$\pm$0.18 & 25.21$\pm$0.39 & 64.03 \\
& Our model w/o msg (2-head decoder) & 64.0$\pm$0.21 & 33.45$\pm$1.22 & 47.65$\pm$0.37 & 26.02$\pm$1.08 & 64.03 \\

& Our model (Argmax Test) & 75.89$\pm$0.24 & 46.08$\pm$0.29 & 61.86$\pm$0.33 & 37.29$\pm$0.36 & 64.28 \\
& Our model (2-head decoder)& 75.36$\pm$0.25 & 44.39$\pm$0.06 & 61.08$\pm$0.55 & 36.14$\pm$0.07 & 64.28 \\\midrule
Lower bound & Single Degraded image & 63.42 & 34.57 & 46.14 & 26.83 & \\\bottomrule
\end{tabular}}
\end{table}

